Ultrafast gap dynamics upon photodoping the Mott-insulating phase of a two-dimensional organic charge-transfer salt

We investigate experimentally the ultrafast changes in the spectral response of the Mott insulator $\kappa$-(BEDT-TTF)$_2$Cu[N(CN)$_2$]Cl ($\kappa$-Cl) upon photodoping with intense excitation at 1.6 eV and probing with continuum pulses simultaneously covering both the terahertz and infrared (IR) ranges (from 0 to 0.6 eV). A quantitative analysis of the differential reflectivity using a multi-band Lorentzian model provide absolute changes in spectral weights and objective global time constants for the relaxation vs. temperature. The transient conductivity spectra deduced from the analysis suggest that the transient photoinduced spectral weight is dominated by a progressive closure of the Mott gap with increasing excitation density, i.e. due to changes in the inter-Hubbard-band absorption by the remaining singly occupied states. We critically examine this scenario compared to that proposed previously, whereby the low-energy spectral weight is attributed to a Drude-like response of photoexcited doublons/holons. We also consider the observed slowing down of the relaxation rate with increasing excitation density, and temperature dependence of the initial doublon/holon density in terms of the phonon-mediated gap recombination model.

==> notes.tex <==
\section{Notes}

GS spectra - analysis:
\cite{kornelsen92,sasaki04,faltermeier07,dumm09,elsasser12,tomic13,vlasova09,vlasova2011}

Specifically Fano phonons:
\cite{fano61,kornelsen92,sedlmeier12,elsasser12}

EMV:
\cite{rice80,painelli86,dressel04} % Add more here?

Within pump-probe studies:
\cite{yamakawa21}

Br: \cite{mcguire01,dressel09}

% Additional low-frequency band identified, but in Br single crystal
%\cite{kawakami18}

GS spectra - theory
\cite{vlasova09,merino08,ferber14}

GS transport gap:
% rho(T) and gap term \cite{pinteric15}
% Just the gap term: %\cite{tomic13}

Fermi-liquid
Non-Drude scattering
\cite{ahn22} % NFL, exp. + DFT/DMFT
\cite{fratini21} % Slow fluctuations -> localisation, DDP
\cite{fratini14} % Localisation -> DDP
\cite{deng13} % DDP, incl. doped Mott, but still strong w=0
\cite{berthod13} % Non-Drude but still FL (not non-FL)
\cite{smith01} % Original DS


OP-MIRP
\cite{yamakawa17} % Br on sapphire
\cite{kawakami09} % d-Cl


OP-OP
\cite{tsuchiya19,naito08} 
